Can Cross Encoders Produce Useful Sentence Embeddings?

Cross encoders (CEs) are trained with sentence pairs to detect relatedness. As CEs require sentence pairs at inference, the prevailing view is that they can only be used as re-rankers in information retrieval pipelines. Dual encoders (DEs) are instead used to embed sentences, where sentence pairs are encoded by two separate encoders with shared weights at training, and a loss function that ensures the pair's embeddings lie close in vector space if the sentences are related. DEs however, require much larger datasets to train, and are less accurate than CEs. We report a curious finding that embeddings from earlier layers of CEs can in fact be used within an information retrieval pipeline. We show how to exploit CEs to distill a lighter-weight DE, with a 5.15x speedup in inference time.

==> sections/edited_table.tex <==


\begin{table*}[!th]
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|r|r|r|l|r|r|r|r|} 
       \cline{1-4} \cline{6-9}
        & \multicolumn{3}{c|}{Retrieve} & &\multicolumn{4}{c|}{Retrieve + Rerank} \\ 
               \cline{2-4} \cline{6-9}
               &  \multicolumn{3}{c|}{Hits@10}   & & \multicolumn{2}{c|}{Hits@10}  & \multicolumn{1}{c|}{Speedup (Times)}  \\
Dataset  &  Baseline  &  DE-2 Random  & DE-2 CE  & & DE-2 CE &  Baseline & DE-2 CE & Baseline \\
       \cline{1-4} \cline{6-9}
all nli  & 0.77 & 0.59 & 0.75 &  &\textbf{ 0.84} & 0.83 & 269.40 & 59.32 \\
eli5  & 0.43 & 0.12 & 0.29 &  & 0.43 & 0.49 & 190.41 & 35.11 \\
gooaq  & 0.75 & 0.42 & 0.64 &  & 0.77 & 0.8 & 246.32 & 42.39 \\
msmarco  & 0.95 & 0.81 & 0.89 &  & 0.61 & 0.64 & 171.80 & 33.55 \\
natural questions  & 0.77 & 0.37 & 0.61 &  & \textbf{0.68 }& 0.68 & 55.29 & 10.17 \\
quora duplicates  & 0.68 & 0.48 & 0.65 &  &\textbf{ 0.97} & 0.97 & 148.20 & 28.99 \\
sentence compression  & 0.95 & 0.83 & 0.93 &  & \textbf{0.97 }& 0.96 & 291.76 & 44.41 \\
simplewiki  & 0.97 & 0.93 & 0.97 &  &\textbf{ 0.98 }& 0.98 & 126.99 & 26.27 \\
stsb  & 0.97 & 0.87 & 0.97 &  & \textbf{0.98} & 0.98 & 422.70 & 90.42 \\
zeshel  & 0.28 & 0.13 & 0.24 &  & 0.25 & 0.27 & 20.83 & 4.35 \\
       \cline{1-4} \cline{6-9}
    \end{tabular}
    % }
    \caption{Comparison of CE infused DE. \textbf{Baseline} is a pre-trained DE model.  \textbf{DE-2 Random} is a trained two-layered DE initialized with random initial weights. \textbf{DE-2 CE} is a two-layered DE infused with initial weight from CE as explained in Fig~\ref{fig:dual_cross} and trained similar to DE-2. }
    % \textbf{Retrieve + Rerank}: Columns 5-6 present Accuracy@10 and columns 7-8 present number of documents encoded per sec. Here, the documents retrieved using baseline and our approach are reranked using a CE.}
    \label{tab:comp}
\end{table*} 
